Energy-Efficient Coverage Enhancement of Indoor THz-MISO Systems: An FD-NOMA Approach

Terahertz (THz) communication is gaining more interest as one of the envisioned enablers of high-data-rate short-distance indoor applications in beyond 5G networks. Moreover, non-orthogonal multiple-access (NOMA)-enabled schemes are promising schemes to realize the target spectral efficiency, low latency, and user fairness requirements in future networks. In this paper, an energy-efficient cooperative NOMA (CNOMA) scheme that guarantees the minimum required rate for the cell-edge users in an indoor THz-MISO communications network is proposed. The proposed cooperative scheme consists of three stages: (i) beamforming stage that allocates base-station (BS) beams to THz cooperating cell-center users using analog beamforming with the aid of the cosine similarity metric, (ii) user pairing stage that is tackled using the Hungarian algorithm, and (iii) power allocation stage for both the BS THz-NOMA transmit power and the cooperation power of the cooperating cell-center users, which are optimized sequentially. The obtained results quantify the energy efficiency (EE) of the proposed scheme and shed new light on the performance of multi-user THz-NOMA-enabled networks.

==> DumpFile.tex <==
The main merits of each transceiver design can be summarized as follows; (i) Electronic solutions can generate high transmission power, (ii) photonic solutions are superior to the electronic ones in term of achieving high data rates; as modulating and processing photonic signals are done at very high speeds, (iii) the integrated hybrid solutions can be programmed and efficiently designed for various emerging system-level properties, (iv) plasmonic solutions have compact and reconfigurable array designs, can support large communication bandwidths, and can operate directly at \ac{THz} frequencies; contrary to electronic solutions that generally depend on the up-conversion of microwave signals and to the photonic solutions that depend on the down-conversion of optical signals~\cite{sarieddeen2019next,han2019terahertz}.

%\textcolor{blue}{We should emphasis here that the joint optimization of beamforming-user pairing-and power allocation is computationally involve. In this work, our proposed approach can provide a low complexity solution for the  \ac{EE} maximization problem. Such low complexity solution is needed reduce the processing burden on the indoor \ac{BS} (access point) that usually has low processing power compared to outdoor base-stations.} 

\subsection{Related Work}
Up to the best of the authors' knowledge, there is no existing work that combines multi-user indoor \ac{MISO}-\ac{NOMA} in \ac{THz} band with user-assisted cooperative side-links for coverage enhancement of cell-edge users. Hence, in this subsection, we present the literature contributions that separately tackle conventional downlink \ac{THz}-\ac{NOMA} enabled systems, and (2) energy-efficient user-assisted cooperative-\ac{NOMA} enabled systems.

\noindent (1)~\textit{Conventional Downlink THz-NOMA enabled Systems}:
The amount of work in the \ac{THz}-\ac{NOMA}-enabled networks is still limited~\cite{8824971,9115278,sabuj2020application}. In~\cite{8824971}, in order to maximize the network throughput, the authors solved an optimization problem that involves beamforming, power allocation, and sub-band assignment. Through numerical simulations, the authors demonstrated the superiority of the proposed scheme compared to the THz-OMA counterpart. In~\cite{9115278}, a downlink heterogeneous \ac{THz}-\ac{NOMA} cache-enabled system with imperfect \ac{SIC} is proposed. An \ac{EE} maximization problem that includes user clustering, beamforming, and power allocation is formulated and then solved by dividing the original problem into three sub-problems. Through simulations, the authors show that the proposed enhanced K-means for user clustering and the proposed alternating direction method of multipliers for power allocation can achieve higher \ac{EE} performance for the proposed network. In~\cite{sabuj2020application}, a machine-type communication downlink sub-\ac{THz}-\ac{NOMA} enabled system to enable massive connectivity of devices have been analyzed. An \ac{EE} maximization problem has been solved via unconstrained then constrained optimization. Through simulations, the authors show that the proposed system attains better performance compared to its counterpart in the mmWave band.

\noindent (2)~\textit{Energy-efficient user-assisted cooperative-\ac{NOMA} enabled systems}:
One can find the works that investigated \ac{EE}-optimal user-assisted cooperative-\ac{NOMA} enabled systems for \ac{SISO} setup in~\cite{8430576,8643955} and \ac{MISO} setup in~\cite{8704259}. Noting that the analysis in the three aforementioned works (i) have been done in sub-$6$ GHz channels, which have different propagation characteristics compared to \ac{THz} channels that is investigated in this work, (ii)  a two-user setup has been analyzed there compared to the multi-user setup that is investigated in this work. 





%Not included figures

%\begin{figure}[!t]
%    \centering
%    \vspace*{-.02in}
%    \subfloat[Frequency window 1 to frequency window 10.]{
%        \hspace*{-.1in}
%        \includegraphics[scale=0.35]{Simulation/I_Changing_Freq_band_f1_f10.eps}
%        \label{fig:f1_f10}
%    }
    %\vspace*{-.14in}
%    \hfill
%  \subfloat[Zoomed version: frequency window 5 to frequency window 10.]{
%        \hspace*{-.1in}
%        \includegraphics[scale=0.35]{Simulation/I_Changing_Freq_band_f5_f10.eps}
%        \label{fig:f5_f10}
%    }
%    \caption{The achievable \ac{EE} performance of the system while changing \ac{THz} potential channel windows. ($p_k$= $5$ Watt, $R_{0}^{\textnormal{min}}$=  $10$ Gbps, $N=4$)}
%\label{fig: potential channel windows}
%\vspace{-1em}
%\end{figure}

%In~\cite{singh2020analytical}, a sensitivity analysis for ten prospective frequency windows in the \ac{THz} spectrum has conducted. In Fig.~\ref{fig:f1_f10}, we evaluated the \ac{EE} performance of the network with those prospective frequency windows. As discussed in the introduction, the operation on \ac{THz} frequency bands comes at the cost of high propagation losses and as the center frequency of the \ac{THz} band increases the path loss becomes more severe, eventually, the sum rate as well as \ac{EE} of the network descend to low levels, this trend is depicted in Fig.~\ref{fig:f1_f10}. To satisfy the ever-increasing bandwidth demands for the newly emerging data-demanding applications, with the current technology nowadays, it is advisable in an indoor environment to operate on the first four prospective frequency windows to achieve large network \ac{EE} with relatively moderate path  loss. 

%\begin{figure}[t!]
%\centering
%\vspace{-1em}
%\includegraphics[scale=0.35]{Simulation/I_Changing_Freq_band_f1_f10.eps}
%\caption{The achievable \ac{EE} performance of the system while changing \ac{THz} potential channel windows. ($p_k$= $5$ Watt, $R_{0}^{\textnormal{min}}$=  $10$ Gbps, $N=4$)}
%\label{fig:f1_f10}
%\vspace{-1.5em}
%\end{figure}

%\begin{figure}[t!]
%\centering
%\vspace{-1em}
%\includegraphics[scale=0.35]{Simulation/F_Changing_min_QoS_EE.eps}
%\caption{The achievable \ac{EE} performance of the system while changing the users minimum required rate, $R_{0}^{\textnormal{min}}$. ($p_k$= $5$ Watt, $N=4$, $f$= $3.42$ THz, $B$= $137$ GHz, $k_{\textnormal{abs}}(f)=14.0 \times 10^{-4} \textnormal{m}^{-1}$)}
%\label{fig: changing R0}
%\vspace{-0.5em}
%\end{figure}
